Continuum Limit of $B_K$ from 2+1 Flavor Domain Wall QCD

We determine the neutral kaon mixing matrix element $B_K$ in the continuum limit with 2+1 flavors of domain wall fermions, using the Iwasaki gauge action at two different lattice spacings. These lattice fermions have near exact chiral symmetry and therefore avoid artificial lattice operator mixing. We introduce a significant improvement to the conventional NPR method in which the bare matrix elements are renormalized non-perturbatively in the RI-MOM scheme and are then converted into the MSbar scheme using continuum perturbation theory. In addition to RI-MOM, we introduce and implement four non-exceptional intermediate momentum schemes that suppress infrared non-perturbative uncertainties in the renormalization procedure. We compute the conversion factors relating the matrix elements in this family of RI-SMOM schemes and MSbar at one-loop order. Comparison of the results obtained using these different intermediate schemes allows for a more reliable estimate of the unknown higher-order contributions and hence for a correspondingly more robust estimate of the systematic error. We also apply a recently proposed approach in which twisted boundary conditions are used to control the Symanzik expansion for off-shell vertex functions leading to a better control of the renormalization in the continuum limit. We control chiral extrapolation errors by considering both the NLO SU(2) chiral effective theory, and an analytic mass expansion. We obtain $B_K^{\msbar}(3 GeV) = 0.529(5)_{stat}(15)_\chi(2)_{FV}(11)_{NPR}$. This corresponds to $\hat{B}_K = 0.749(7)_{stat}(21)_\chi(3)_{FV}(15)_{NPR}$. Adding all sources of error in quadrature we obtain $\hat{B}_K = 0.749(27)_{combined}$, with an overall combined error of 3.6%.

==> AuthorsAbstractTitle <==
 
Y. Aoki, R. Arthur, T. Blum, P.A. Boyle,D. Br\"ommel, N.H. Christ, 
C. Dawson, T. Izubuchi, C. Jung, C. Kelly, R.D. Kenway, M. Lightman,
R.D. Mawhinney, Shigemi Ohta, C.T. Sachrajda, 
E.E. Scholz, A. Soni, C. Sturm, J. Wennekers, and R. Zhou

Continuum Limit of $B_K$ from 2+1 Flavor Domain Wall QCD


We determine the neutral kaon mixing matrix element $B_K$
in the continuum limit with 2+1 flavors of domain wall fermions,
using the Iwasaki gauge action at two different lattice spacings.  
These lattice fermions have near exact chiral symmetry and 
therefore avoid artificial lattice operator mixing.

We introduce a significant improvement to the conventional NPR method in which the 
bare matrix elements are renormalized non-perturbatively in the RI-MOM scheme 
and are then converted into the $\overline{\textrm{MS}}$ scheme using continuum 
perturbation theory. In addition to RI-MOM, we introduce and implement four non-exceptional 
intermediate momentum schemes that suppress infrared non-perturbative uncertainties 
in the renormalization procedure. We compute the conversion factors relating the matrix elements 
in this family of RI-SMOM schemes
and $\overline{\textrm{MS}}$ at one-loop order. Comparison of the results obtained using these
different intermediate schemes allows for a more reliable estimate of the unknown higher-order
contributions and hence for a correspondingly more robust estimate of the systematic error. 
We also apply a recently proposed approach in which twisted boundary conditions are used to 
control the Symanzik expansion for off-shell vertex functions 
leading to a better control of the renormalization in the continuum limit.

We control chiral extrapolation errors by considering both the NLO
SU(2) chiral effective theory, and an analytic mass expansion.
We obtain $B_K^{\overline{\mathrm{MS}}}(3\,\mathrm{GeV}) = 0.529(5)_\mathrm{stat}(15)_\chi(2)_{\mathrm{FV}}(11)_{\mathrm{NPR}}$.
This corresponds to $\hat{B}_K^{\overline{\mathrm{RGI}}} = 0.749(7)_\mathrm{stat}(21)_\chi(3)_{\mathrm{FV}}(15)_{\mathrm{NPR}}$.
Adding all sources of error in quadrature we obtain
$\hat{B}_K^{\overline{\mathrm{RGI}}} = 0.749(27)_{\mathrm{combined}}$, 
with an overall combined error of 3.6\%.


==> tab/combinedfpsresults.tex <==
\begin{table}
\centering
\begin{tabular}{c|ccc}
\hline
Fit & $f_\pi$ (GeV) & $f_K$ (GeV) & $f_K/f_\pi$\\
\hline
NLO PQChPT & $0.117(2)$ & $0.144(2)$ & $1.233(8)$\\
NLO PQChPT+FV & $0.119(2)$ & $0.145(2)$ & $1.219(7)$\\
LO Analytic & $0.124(2)$ & $0.148(2)$ & $1.196(8)$\\
\hline
PDG Physical & $0.1304(2)$ & - & - \\
\end{tabular}
\caption{Predicted pion and kaon decay constants obtained from our combined 
analysis using NLO PQChPT and LO analytic fit forms. The second line contains 
the results to an NLO PQChPT fit including finite volume corrections. Errors are statistical 
only. The physical value of $f_\pi^-$ is obtained from the 2009 PDG review\cite{Amsler:2008zzb}.
\label{tab:combinedfpsresults}} 
\end{table}
%PDG Physical & $0.1304(2)$ & $0.1555(9)$ & $1.193(6)$

